SeaLLMs -- Large Language Models for Southeast Asia

Despite the remarkable achievements of large language models (LLMs) in various tasks, there remains a linguistic bias that favors high-resource languages, such as English, often at the expense of low-resource and regional languages. To address this imbalance, we introduce SeaLLMs, an innovative series of language models that specifically focuses on Southeast Asian (SEA) languages. SeaLLMs are built upon the Llama-2 model and further advanced through continued pre-training with an extended vocabulary, specialized instruction and alignment tuning to better capture the intricacies of regional languages. This allows them to respect and reflect local cultural norms, customs, stylistic preferences, and legal considerations. Our comprehensive evaluation demonstrates that SeaLLM-13b models exhibit superior performance across a wide spectrum of linguistic tasks and assistant-style instruction-following capabilities relative to comparable open-source models. Moreover, they outperform ChatGPT-3.5 in non-Latin languages, such as Thai, Khmer, Lao, and Burmese, by large margins while remaining lightweight and cost-effective to operate.

==> Sbackground.tex <==
\section{Related Work}\label{sec:rel_works}



% plot chart but log scale
\makeatletter
% \newcounter{groupcount}
\pgfplotsset{
  col chart axis style/.style={
    width=\columnwidth,
    height=0.15\textheight,
    xtick=data,
    enlarge y limits=false,
    enlarge x limits=0.05,
  },
  col bar axis style/.style={
    col chart axis style,
    % ylabel=Accuracy (\%),
    % xticklabels=\empty,
    % xticklabels from table={\dataA}{[index] 0},
    % x tick label style={yshift={-0.1}},
    % xticklabel style={text height=1ex},
    % xticklabels from table={\dataindic}{[index] 1},
    enlarge y limits=false,
    enlarge x limits=0.05,
    ymin=40, 
    ymax=65,
    ybar=0.1em,
    bar width=9pt,
    legend style={
      font=\footnotesize,
      % cells={anchor=west},
      legend columns=2,
      % at={(0.5, -0.05)},  % position of the anchor: relateive to axis, right 0.5 portion, below 0.05 portion
      at={(0.15, 0.95)},  % position of the anchor: relateive to axis, right 0.5 portion, below 0.05 portion
      % at={(0.3,-0.25)},
      % pos=north west,
      anchor=north, % the anchor: which side of the legend `at` is at
      /tikz/every even column/.append style={column sep=0.5cm},
    },
  },
}

% TOO MUCH WORDS, must reduce, if submit to conference

% large language models, in-context learning
Large language models (LLMs) display outstanding capabilities because they are pre-trained on massive amounts of internet text data \citep{gpt3_brown2020language,palm_chowdhery2022palm,bloom_scao2022bloom,llama_touvron2023,llama2_touvron2023llama}. Without any gradient update, base LLMs are able to perform in-context learning by simply observing a list of high-quality input-output exemplars \citep{gpt3_brown2020language,llm_do_icl_differently_wei2023larger}. This technique works across many tasks that involve language understanding, reasoning and generation \citep{gpt3_brown2020language,cot_wei2022chain,llm_are_mling_cot_shi2022language}. Much research has been conducted to understand in-context learning. 
Some suggest that the models secretly perform gradient descent on the exemplars \citep{icl_gradient_descen_dai2022can}, while others demonstrate that most of the knowledge is learned during pre-training, and the exemplars are only to provide evidence for the model to \textit{locate} the intended task via a Bayesian inference process \citep{icl_bayesian_infer_xie2021explanation,rethink_demonstration_min2022rethinking,lima_zhou2023lima}.

% : \joty{we can exclude the Eq, if needed}
% \begin{equation}
%     p(y|\text{x}) = \int_{\text{task}} p(y|\text{task,x})p(\text{task}|\text{x})d(\text{task})\label{eqn:prompt_concept}
% \end{equation}

% TODO: consider move this to appendix
% \begin{figure}[h]
%     \centering
%     \begin{tikzpicture}
%     \begin{axis}[
%       col bar axis style,
%       % xticklabels from table={\dataindic}{[index] 1},
%       % ylabel=\%,
%     %   xticklabels from table={\langpercent}{lang},
%       xticklabels={,,},
%       xtick=\empty,
%       ymin=0.00001, 
%       ymax=1,
%       ybar=0.1em,
%       bar width=3pt,
%     %   ytick distance=.5,
%     %   log basis y={10},
%       ymode=log,
%       log origin y=infty,
%     ]
%       \addplot table[x=id, y=percent ] \langpercentafrican;
%     %   \addplot table[x=id, y=percent ] \langpercent;
%       \addplot table[x=id, y=percent ] \langpercentindic;
%     %   TODO: we should use total table langpercent but add data truncat data differently
%       \legend{African, Indic}
%     \end{axis}
%     \end{tikzpicture}
%     \caption{Low-resource language coverage \% of the ROOTS corpus \citep{roots_corpus} used to train BLOOM. The highest-resource language for Indic and African are Hindi and Swahili. Hindi accounts for $0.7$\% and the rarest language, Tumbuka, takes up only $2e^{-5}$\% of the corpus.}
%     \label{fig:bloom_lang_coverage}
% \end{figure}


% and multilingual , polyglot fine-tuning
% even if these make up a tiny fraction of the largely English corpora
Most LLMs are trained with multilingual corpora \citep{ccnet_wenzek-etal-2020-ccnet}, even if these make up a tiny fraction of the large English corpora \citep{gpt2_radford2019language_gpt2,gpt3_brown2020language}. Despite that, LLMs still exhibit strong multilingual capabilities with high-resource languages like French, German and Chinese, often with the help of English-pivoting using supervised translation systems \citep{llm_are_mling_cot_shi2022language} or prompting the model to firstly generate intermediate English context \citep{xlt_not_all_created_equal_huang2023not}. 
% The most multilingual LLM is BLOOM \citep{bloom_scao2022bloom}, which was trained on 46 languages of the ROOTS corpus \citep{roots_corpus}, including 34 Indic and African languages that can be considered low-resource, and having a pre-training coverage from less than 1\% in Hindi for Indic group to $2e^{-5}$\% in Tumbuka for African group, as shown in \Cref{fig:bloom_lang_coverage}. 
% One ofThe most \joty{what?} multilingual LLM is BLOOM \citep{bloom_scao2022bloom}, which was trained on 46 languages in the ROOTS corpus \citep{roots_corpus}. 
BLOOM \citep{bloom_scao2022bloom} is one of the LLMs trained with the most number of languages, whose ROOTS corpus consists of data from 46 languages \citep{roots_corpus}. 
The ROOTS corpus includes 34 Indic and African languages regarded as low-resource, with each language having a pre-training coverage of less than 1\% in Hindi for the Indic group, to $2e^{-5}$\% in Tumbuka for the African group, as shown in \Cref{fig:bloom_lang_coverage} in the Appendix. 
% \joty{The previous sent needs revision.}????
% Interestingly, some common high-resource languages, such as Russian, were not used in the training of BLOOM, making it a good subject to study unseen languages. 
% We use BLOOM as the main model to evaluate our methods and baselines in the 34 low-resource languages. 
Exclusively only for unsupervised translation tasks, our linguistically-diverse prompting (LDP) strategy is also an English-pivoting method, but it is different from other cross-lingual counterparts \citep{llm_are_mling_cot_shi2022language,xlt_not_all_created_equal_huang2023not} in that while others only pivot inputs to English intermediates, we use in-context pairs between English and a diverse set of high-resource languages to promote the intended task in the target low-resource language. For other intra-lingual tasks like instruction following, where input and output are both expected to be in the same language, our LDP helps prevent English-tuned models \citet{llama2_touvron2023llama} from responding with English answer given a non-English query.

% ...Russian, were not used in the training of BLOOM, making it...

% The most multilingual LLM is BLOOM \citep{bloom_scao2022bloom}, which was trained on 46 languages in the ROOTS corpus \citep{roots_corpus}. The ROOTS corpus includes 34 Indic and African languages regarded as low-resource, and having a pre-training coverage of less than 1\% in Hindi for the Indic group, to $2e^{-5}$\% in Tumbuka for the African group, as shown in \Cref{fig:bloom_lang_coverage}. 
% The most multilingual LLM is BLOOM, which was trained on 46 languages in the ROOTS corpus. The ROOTS corpus includes 34 Indic and African languages regarded as low-resource, and having a pre-training coverage of less than 1\% in Hindi for the Indic group, to $2e^{-5}$\% in Tumbuka for the African group, as shown in \Cref{fig:bloom_lang_coverage}


Part of our work also intersects with unsupervised multilingual machine translation (UMT), where back-translation is proven to be effective \citep{understanding_backtranslation_scale,lample2018phrase_unsup,conneau2019cross_xlm,mbart_liu2020multilingual,refine_lowres_umt_nguyen2022}, along with other methods \citep{criss2020,swavumt_nguyen2022contrastive}. English-pivoting is also prominent in the realm of machine translation, where training models on high-resource En$\leftrightarrow$X bitext improves lower-resource En$\leftrightarrow$Y tasks \citep{multilingual_view_garcia-etal-2020,harness-multilingual-garcia-etal-2021}. 
% Nonetheless, the noteworthy gap between existing UMT and LLMs is that their language coverages do not overlap much, preventing us from using UMT models to enhance LLMs. For example, BLOOM does not cover 14 languages supported by CRISS \citep{criss2020}.
Analyses of machine translation using LLMs have also been done. \citet{howgood_gpt_mt_hendy2023good} show that GPT models can perform competitively alongside the best MT models. \citet{mmt_llm_analysis_zhu2023multilingual} focus on optimizing supervised exemplars selection strategies, while \citet{icl_maintain_coherence_sia2023context} discover that using specific coherent prompts for each input helps improve performance. Nonetheless, such studies only consider supervised instruction-tuned models \citep{instructgpt_ouyang2022training,bloomz_muennighoff2022crosslingual}, which may risk test-set contamination \citep{bloomz_muennighoff2022crosslingual}. Thus, there is still limited research involving low-resource languages in completely zero-shot setups. 
As such, since low-resource languages may not enjoy the privilege of having large unlabeled data to conduct searching, only random selection is used in this study, while optimal exemplar selection is out of scope.



% Meanwhile, optimal exemplar selection is not within the scope of this paper and we only use random selection as low-resource languages may not enjoy the privilege of having large unlabeled data to conduct searching.

% Should reverse the order of information --- [because of Low-res having low data] we have to exclude optimal exemplars & use random selection.% Revise to:


% if have space, mention
% multilingual translation, mbart, mbart50, NLLB
% translation with large language models, how good gpt at, choice of prompt, maintain coherence  (document-level translation)
% combination of both: english pivotting, in LLMs and other literatures of MT
% TODO: synthetic prompt generation and gneeering?







% \citep{data_diversification2020}
% \citep{cbd_nguyen2021}
% \citep{swavumt_nguyen2022contrastive}
% \citep{refine_lowres_umt_nguyen2022}

% \citep{cot_wei2022chain}
% \citep{llm_are_mling_cot_shi2022language}
% \citep{mmt_llm_analysis_zhu2023multilingual}
% \citep{icl_maintain_coherence_sia2023context}
% \citep{how_good_gpt_mt_hendy2023good}
% \citep{self_refine_madaan2023self}

% \citep{polyglot-fu-etal-2022-polyglot}

% \citep{levenshtein1966binary}
% \citep{nllb_costa2022no_flores200}
% \citep{swav_caron2020unsupervised}
% \citep{gpt3_brown2020language}
% \citep{palm_chowdhery2022palm}
% \citep{llama_touvron2023}
% \citep{bloom_scao2022bloom}
% \citep{howgood_gpt_mt_hendy2023good}
% \citep{prompt_llm_mt_casestudy_zhang2023prompting}
% \citep{opt175b_zhang2022opt}
% \citep{fewshot_multilingual_winata2021language}

% \citep{param_share_multilingual_sachan-neubig-2018}
% \cite{cbd_nguyen2021}
% \citep{data_aug_low_resource_fadaee-etal-2017-data}
% \citep{bloomz_muennighoff2022crosslingual}
% \citep{bloom_scao2022bloom}
% \citep{refine_lowres_umt_nguyen2022}








